Large-scale Multi-label Learning with Missing Labels

The multi-label classification problem has generated significant interest in recent years. However, existing approaches do not adequately address two key challenges: (a) the ability to tackle problems with a large number (say millions) of labels, and (b) the ability to handle data with missing labels. In this paper, we directly address both these problems by studying the multi-label problem in a generic empirical risk minimization (ERM) framework. Our framework, despite being simple, is surprisingly able to encompass several recent label-compression based methods which can be derived as special cases of our method. To optimize the ERM problem, we develop techniques that exploit the structure of specific loss functions - such as the squared loss function - to offer efficient algorithms. We further show that our learning framework admits formal excess risk bounds even in the presence of missing labels. Our risk bounds are tight and demonstrate better generalization performance for low-rank promoting trace-norm regularization when compared to (rank insensitive) Frobenius norm regularization. Finally, we present extensive empirical results on a variety of benchmark datasets and show that our methods perform significantly better than existing label compression based methods and can scale up to very large datasets such as the Wikipedia dataset.

==> analysis.tex <==
\section{Generalization Error Analysis for Missing Labels}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "nips2013"
%%% End: 


==> format-and-defs.tex <==
%\usepackage{amsmath,amssymb,amsthm}
%\usepackage{fullpage}
%\usepackage{setspace}
%\usepackage{tabularx}
%\usepackage{caption}
%\usepackage{xcolor}
%\usepackage{algorithm,algorithmic}
%\usepackage{rotating}
%\usepackage{fancyhdr}
%\usepackage{stmaryrd}
%\usepackage{subcaption}
%\usepackage{array}
%\usepackage{dsfont}
%\usepackage{appendix}
%\usepackage[round,sort]{natbib}
%\usepackage{lettrine}
%\usepackage{url}
%\usepackage{float}
%\usepackage{pdflscape}
%\usepackage{enumerate}

% NIPS 2012 definitions

\newtheorem{lem}{Lemma}
\newtheorem{thm}[lem]{Theorem}
\newtheorem{cor}[lem]{Corollary}
\newtheorem{clm}[lem]{Claim}
\newtheorem{defn}[lem]{Definition}
\newtheorem{fact}[lem]{Fact}
\newtheorem{obs}[lem]{Observation}

\newcommand{\R}{{\mathbb R}}
\newcommand{\RR}{{\cal R}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\cn}[2]{{\cal N}_{#1}\br{#2}}
\renewcommand{\H}{{\cal H}}
\newcommand{\X}{{\cal X}}
\newcommand{\D}{{\cal D}}
\renewcommand{\L}{{\cal L}}
\newcommand{\T}{{\cal T}}
\newcommand{\Y}{{\cal Y}}
\newcommand{\A}{{\cal A}}
\newcommand{\F}{{\cal F}}
\newcommand{\W}{{\cal W}}
\newcommand{\Q}{{\cal Q}}
\renewcommand{\P}{{\cal P}}

\newcommand{\bc}[1]{\left\{{#1}\right\}}
\newcommand{\br}[1]{\left({#1}\right)}
\newcommand{\bs}[1]{\left[{#1}\right]}
\newcommand{\abs}[1]{\left| {#1} \right|}
\newcommand{\norm}[1]{\left\| {#1} \right\|}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\bsd}[1]{\left\llbracket{#1}\right\rrbracket}

\newcommand{\etal}{\emph{et al}\ }
\renewcommand{\O}[1]{{\cal O}\br{{#1}}}
\newcommand{\softO}[1]{\tilde{\cal O}\br{{#1}}}
\newcommand{\Om}[1]{\Omega\br{{#1}}}
\newcommand{\E}[1]{{\mathbb E}\bsd{{#1}}}
\newcommand{\EE}[2]{\underset{#1}{\mathbb E}\bsd{{#2}}}
\newcommand{\usup}[1]{\underset{#1}{\sup}}
\newcommand{\uinf}[1]{\underset{#1}{\inf}}
\newcommand{\Var}[1]{\text{Var}\bsd{{#1}}}
\renewcommand{\Pr}[1]{{\mathbb P}\bs{{#1}}}
\newcommand{\Prr}[2]{\underset{#1}{\mathbb P}\bs{{#2}}}
\newcommand{\ip}[2]{\left\langle{#1},{#2}\right\rangle}

\renewcommand{\vec}[1]{{\mathbf{#1}}}
\newcommand{\vecx}{\vec{x}}
\newcommand{\x}{\vecx}
\newcommand{\vecy}{\vec{y}}
\newcommand{\vecz}{\vec{z}}
\newcommand{\vecxy}{\vecx,\vecy}
\newcommand{\vecw}{\vec{w}}
\newcommand{\vecW}{\vec{W}}
\newcommand{\veco}{\boldsymbol\omega}
\newcommand{\vecr}{\vec{r}}
\newcommand{\vecs}{\vec{s}}
\newcommand{\vecv}{\vec{v}}
\newcommand{\veczero}{\vec{0}}
\newcommand{\vectheta}{\text{\boldmath$\theta$}}

\newcommand{\eil}[2]{\ell_{#1}\br{#2}}
\newcommand{\eild}[1]{\eil{\epsilon}{#1}}
\newcommand{\ellac}[2]{\eil{\text{actual}}{#1,#2}}
\newcommand{\gml}[2]{\bs{#2}_{#1}}
\newcommand{\gmld}[1]{\gml{\gamma}{#1}}
\newcommand{\pos}[1]{\gml{+}{#1}}
\newcommand{\evbad}[1]{\textsf{BAD-APPROX}\br{#1}}
\newcommand{\st}{\mathop{\text{subject to}}}
\newcommand{\lord}[1]{\ell_{\text{ord}}\br{#1}}
\newcommand{\lndcg}[1]{\ell_{\text{NDCG}}\br{#1}}
\newcommand{\pmone}{\bc{-1,+1}}
\newcommand{\ind}{\mathds{1}}
\newcommand{\lsq}[1]{\ell_{\text{sq}}\br{#1}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

% NIPS 2011 definitions

\newcommand{\B}{{\cal B}}
\newcommand{\Nr}{{\cal N}}
\newcommand{\sgn}{\mathop{\text{sgn}}}
\newcommand{\id}{\mathop{\text{id}}}
\newcommand{\bad}[1]{\mathsf{BAD}\br{#1}}
\newcommand{\ftune}{{\bf FTUNE}}
\newcommand{\ftunei}{{\bf FTUNE+D}}
\newcommand{\bbs}{{\bf BBS}}
\newcommand{\dboost}{{\bf DBOOST}}
\newcommand{\bbsi}{{\bf BBS+D}}
\newcommand{\dselect}{{\bf DSELECT}}
\newcommand{\rand}{\textsc{get-random-element}}
\newcommand{\train}{\textsc{train}}

% AISTATS 2012 definitions

\newcommand{\Hone}{\textbf{H0/1}}
\newcommand{\RF}{\textbf{RF}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\Kc}{K_{\text{co}}}
\newcommand{\Kip}{K_{\text{dp}}}
\newcommand{\ball}[3]{{\cal B}_{#1}\br{{#2},{#3}}}
\newcommand{\loneunitball}{\ball{1}{\vec{0}}{1}}
\newcommand{\loneball}[1]{\ball{1}{\vec{0}}{#1}}
\newcommand{\ltwounitball}{\ball{2}{\vec{0}}{1}}
\newcommand{\ltwoball}[1]{\ball{2}{\vec{0}}{#1}}
\newcommand{\lpball}[2]{\ball{{#1}}{\vec{0}}{#2}}
\newcommand{\error}{{\cal E}}
\newcommand{\Nz}{\N \cup \{0\}}

% Bochner definitions

\newcommand{\vect}{\vec{t}}
\newcommand{\vecone}{\vec{1}}
\newcommand{\ZZ}{{\mathbb Z}}
\renewcommand{\th}{^{\text{th}}}

% Homogeneous definitions

\newcommand{\nR}{{\mathbb R}^{\times}}
\newcommand{\sign}[1]{\text{sign}\br{#1}}

% Intro definitions

\newcommand{\C}{{\cal C}}
\newcommand{\Z}{{\cal Z}}

% ICML 2013 definitions

\newcommand{\rk}{{\mathfrak r}}
\newcommand{\Rk}{{\mathfrak R}}
\newcommand{\Vk}{{\mathfrak V}}
\newcommand{\Wk}{{\mathfrak W}}
\newcommand{\Dk}{{\mathfrak D}}

\newcommand{\mrs}{{\bfseries RS-x }}
\newcommand{\mmrs}{{\bfseries RS-x$\mathbf{^2}$ }}
\newcommand{\rsorig}{{\bfseries RS }}
\newcommand{\olp}{{\bfseries OLP }}
\newcommand{\Lbuft}{\hat\L^{\text{buf}}_t}
\newcommand{\Ltbuft}{\tilde\L^{\text{buf}}_t}
\newcommand{\Rkbufn}{\Rk_n^{\text{buf}}}

\newcommand{\vecmu}{\boldsymbol\mu}
\newcommand{\M}{{\cal M}}
\newcommand{\vecsigma}{\boldsymbol\sigma}
\newcommand{\vecX}{\vec{X}}

% New commands multilabel
\newcommand{\K}{{\cal K}}
\newcommand{\event}{{\cal E}}
\renewcommand{\S}{{\cal S}}
\newcommand{\U}{{\cal U}}
\newcommand{\vecl}{\vec{l}}
\newcommand{\veceps}{\text{\boldmath$\epsilon$}}
\newcommand{\vecdel}{\text{\boldmath$\delta$}}
\newcommand{\tr}[1]{\text{tr}\br{#1}}

==> kernel_extent.tex <==
\section{Kernel Extension}
\label{sec:kernel}
\vspace{-1em}
Given a kernel function $\cK(\cdot,\cdot)$, we can consider 
that $f^{j} \in \cH_{\cK}$ is a function in the corresponding reproducing 
kernel Hilbert space. By Representer Theorem, the minimizer $f^j$ for any risk 
function such as the empirical loss defined in Eq. \eqref{eq:erm} and \eqref{eq:erm_missing} 
admits a representation the form:
\begin{align*}
  f^j(\cdot;\z_j) = \sum_{t=1}^{n} z_{tj} \cK(\cdot, \x_t),
\end{align*}
where $\z_{j} \in \cR^n$.  Let the vector function 
$\kk(\x): \cR^d \rightarrow \cR^n$ for $\cK$ is defined by 
\begin{align*}
\kk(\x) = [\cdots, \cK(\x, \x_t), \cdots]^T.
\end{align*}
Then $f(\x; Z)$ can be written as $f(\x; Z) = Z^T \kk(\x)$, where 
$Z$ is an $n\times L$ matrix with $z_j$ as the $j$-th column. 
Once again, we can impose the same trace norm regularization $r(Z)$ and the low rank 
constraint in Eq. \eqref{eq:erm_W_H}. As a result, $Z= WH^T$ and 
$f^j(\x_i, \z_j) = \kk^T(\x_i) W \h_j$. Assume $K$ is the kernel matrix for 
the training set $\{\x_i\}$ and $K_i$ is the $i$-th column. Then the loss in \eqref{eq:erm_W_H} 
can be replaced by $\l(Y_{ij}, K_i^T W \h_j)$. Thus, the proposed alternating 
minimization can be applied to solve Eq. \eqref{eq:erm} and 
\eqref{eq:erm_missing} with kernel extension. 

%
%By Representer Theorem, 
%In this section, we study multi-label classification in a principled and generic 
%framework. Let $(X,Y)=\{(\x_1, \y_1), (\x_2, \y_2), \dots, (\x_n, \y_n)\}$ be 
%the given training set where 
%$X=[\x_1\ \x_2\ \dots\ \x_n]^T,\ Y=[\y_1\ \y_2\ \dots\ \y_n]^T$,  
%$\x_i\in \R^{d}$ is the $i$-th data point's feature vector, 
%$\y_i \in \{0, 1\}^L$ is the $i$-th data point's label vector with $L$ labels.  
%
%
%Let $Y_{ij}$ denote the $j$-th label of the $i$-th data point, where $Y_{ij}=1$ 
%denotes the label being ``on'' and $Y_{ij}=0$ denotes the label being 
%``absent'' or ``off''.  In this paper, we will consider both these cases. Note 
%that, in this paper we focus mostly on the binary  
%classification setting, but our methods can be easily extended to the multi-class 
%setting where each label $Y_{ij} \in \{1, 2, \dots, C\}$.  
%
%Let $\ell(\y, f(\x; Z))\in \R$ be the loss function that computes 
%discrepancy between the ``true'' label vector $\y$ and the prediction 
%$f(\x; Z)$ that is parameterized by  $Z\in \mathbb{R}^{d\times L}$. Here, we 
%assume the loss function to be decomposable, i.e., 
%$\ell(\y, f(\x; Z))=\sum_{j=1}^L \ell(y^j, f^j(\x; Z))$ where $y^j$ denotes the $j$-th 
%coordinate of $\y$. Furthermore, we present our results for the linear case of 
%$f(\x; Z)=Z^T\x$; our results can be easily extended to non-linear kernels as 
%well.  
%
%Now, in typical large scale multi-label classification problems, the number of 
%labels is very large but they are heavily correlated and hence can be captured 
%by a significantly smaller number of parameters than $d\cdot L$. In this paper, 
%we assume that the parameter matrix $Z$ learns a small number of ``latent'' 
%factors and hence is a low-rank matrix. This assumption not only enables our 
%methods to control overfitting but also helps in making them computationally 
%efficient.  
%
%Given the training set $(X, Y)$ and the loss function $\ell$, we propose to 
%learn parameters $Z$ by using the canonical regularized empirical risk 
%minimization (ERM) method, i.e.,  
%\begin{equation}
%  \label{eq:erm}
%  \hat{Z}=\arg \min_{Z} J(Z)=\sum_{i=1}^n \sum_j \ell(Y_{ij}, f^j(\x_i; Z)) + \lambda\cdot r(Z), \ \ \ s.t.\ \  \rank(Z)\leq k,
%\end{equation}
%where $r(Z): \R^{d\times L}\rightarrow \R$ is the regularization function. 
%Furthermore, in the presence of missing labels, we compute loss over only the 
%known labels, i.e., 
%\begin{equation}
%  \label{eq:erm_missing}
%  \hat{Z}=\arg\min_{Z} J_\Omega(Z)=\sum_{i=1}^n \sum_{(i,j)\in \Omega}\ell(Y_{ij}, f^j(\x_i; Z)) + \lambda\cdot r(Z), \ \ \ s.t.\ \  \rank(Z)\leq k,
%\end{equation}
%where $\Omega \in [1:n]\times [1:L]$ is the index set that represents 
%``known'' labels. Note that in this work, we are in the standard missing value 
%setting, where each label can be either positive, negative (i.e., $Y_{ij}=1$ or 
%$0$), or missing ($Y_{ij}=?$); several other researches have considered another 
%setting where only positive labels are known and are given as $1$ in the label 
%matrix, while negative or missing values are all denoted by $0$ \cite{RA13a,SSB11a}.
%
%Note that the above generic formulation is NP-hard in general due to the non-convex rank constraint. However, assuming the loss function to be convex, one can derive standard alternating minimization method.  %for such problems that perform  reasonably well in practice and have been shown to be globally optimal in certain settings as well \cite{JainNS13}. 
%Moreover, for the special case of $L_2$ loss,  we can derive closed form solutions for the full-label case \eqref{eq:erm} and  show connections to several existing methods. 
%%In this paper, we study general convex loss functions $\ell$, 
%%Note, that for the special case of squared error loss, i.e., $\ell(\y, f(\x; Z))=\|\y-f(\x;Z)\|_2^2$ 
%\subsection{Special Case: Squared-$L_2$ loss}\label{sec:l2full}
%In this section, we study \eqref{eq:erm} and \eqref{eq:erm_missing} for the 
%special case of squared $L_2$ loss function, i.e., 
%$\ell(\y, f(\x; Z))=\|\y-f(\x;Z)\|_2^2$. We show that in the full-label case 
%(i.e., no missing labels), \eqref{eq:erm} with $L_2$ loss can be solved 
%optimally using SVD. Furthermore, by selecting an appropriate regularizer 
%$r(Z)$ and $\lambda$, our solution for $L_2$ loss is exactly the same as that 
%of \CPLST \cite{YNC12a}.
%
%We first provide closed form solution to \eqref{eq:erm} with 
%$\ell(\y, f(\x; Z))=\|\y- Z^T\x\|_2^2$ and $\lambda= 0$ (i.e., without regularization). 
%\begin{claim}
%  \label{claim:close}
%  If $\ell(\y, f(\x; Z))=\|\y- Z^T\x\|_2^2$ and $\lambda= 0$, then
%  \begin{equation}
%    \label{eq:close}
%    V_{X}\Sigma_{X}^{-1} M_k = \arg\min_{Z: \rank(Z)\leq k} \|Y - XZ\|_F^2,
%  \end{equation}
%  where $X = U_{X} \Sigma_{X} V_{X}^T$ is the thin SVD decomposition of $X$, 
%   and $M_k$ is the rank-$k$ truncated SVD of $M \equiv U_{X}^T Y$.
%\end{claim}
%See Appendix~\ref{app:close} for a detailed proof of Claim \ref{claim:close}. We next 
%show that the above closed form solution is equivalent to the solution 
%provided by the recently proposed \CPLST scheme~\cite{YNC12a}.  
%\begin{claim}\label{claim:cplst}
%  The above closed form solution is equivalent to 
%  $Z^{\text{\CPLST}} = W_{\CPLST} H_{\CPLST}^T$, where $(W_{\CPLST}, H_{\CPLST})$ is the solution provided 
%  by \CPLST, i.e., 
%  \begin{equation}
%    (W_{\CPLST}, H_{\CPLST}) = \arg\min_{\substack{W \in \cR^{d \times k}\\H \in \cR^{L 
%    \times k}}}  \| XW - YH\|_F^2 + \|Y - Y H H^T\|_F^2,\quad s.t.\quad H^TH = I_k.
%    \label{eq:cplst}
%  \end{equation}
%\end{claim}
%See Appendix~\ref{app:close} for a proof. Note that \cite{YNC12a} derives 
%their method by relaxing a Hamming Loss problem and by dropping  
%constraints in the canonical correlation analysis in a relatively ad-hoc 
%manner. However, we show above that the same model can actually be derived  
%in a more principled  manner. This helps us in extending the method in a 
%variety of ways:   
%\begin{compactitem}
%\item As shown empirically, \CPLST tends to overfit significantly whenever 
%  $d$ is large. However, we can handle this issue 
%  by setting the regularization parameter appropriately.  
%
%\item The closed form solution in \cite{YNC12a} cannot directly handle missing 
%  labels as it requires SVD on fully observed $Y$. In contrast, we can handle 
%  missing values under the same framework. 
%%\item The method in \cite{YNC12a} cannot directly handle missing labels as it 
%%  requires computation of the SVD of $X^\dag Y$. On the other hand, we can now 
%%  handle missing values in the same framework. 
%%  %such that in the limit case of no-missing values, our solution is same as \CPLST.  
%  \item The formulation in \cite{YNC12a} is tied to an $L_2$ loss 
%  function. In contrast, we can easily handle other loss functions; although, 
%  the optimization problem might become more difficult to solve.  
%\end{compactitem}
%%%% Local Variables: 
%%%% mode: latex
%%%% TeX-master: "nips2013"
%%%% End: 

